Nonnegative Bayesian nonparametric factor models with completely random measures for community detection

We present a Bayesian nonparametric Poisson factorization model for modeling network data with an unknown and potentially growing number of overlapping communities. The construction is based on completely random measures and allows the number of communities to either increase with the number of nodes at a specified logarithmic or polynomial rate, or be bounded. We develop asymptotics for the number of nodes and the degree distribution of the network and derive a Markov chain Monte Carlo algorithm for targeting the exact posterior distribution for this model. The usefulness of the approach is illustrated on various real networks.

==> intro.tex <==
\section{Introduction}

%Early references on nonnegative matrix factorization \citep{Paatero1994,Lee2001}. Probabilistic versions of NNMF and Poisson factorization models were introduced by \cite{Dunson2005} in the signal processing literature \citep{Virtanen2008,Cemgill2009} and later popularized in the machine learning and physics communities to build network models and recommender systems \citep{Ball2011}.
%
%Related stuff, may not cite. Poisson-gamma regression model (Canny2004)
%
%
%
%Introduce some motivation for the nonnegative matrix factorization here, compared to a probit factor model for example.


Non-negative matrix factorization (NMF) methods~\citep{Paatero1994,Lee2001} and the related Poisson factorization models~\citep{Dunson2005} aim at finding a latent representation of a positive $n\times m$ count matrix $A$ as a sum of $K$ non-negative factors. These methods have found wide applicability in signal processing~\citep{Virtanen2008,Cemgil2009} or recommender systems~\citep{Ma2011,Gopalan2015}. The focus of this paper is on the important application of Poisson factorization to network analysis, where the $n\times n $ count matrix $A$ represents the number of directed or undirected interactions between $n$ individuals, and the latent factors may be interpreted as (potentially overlapping) latent communities~\citep{Ball2011} such as work, sport membership or social activities.\medskip


These approaches require the user to set the number $K$ of latent factors, which is typically assumed to be fixed. To address this problem, \cite{Zhou2012}, \cite{Gopalan2014}, \cite{Zhou2015} and \cite{Ohama2017} proposed Bayesian nonparametric approaches that allow the number of latent factors to be estimated from the data, and to grow unboundedly with the size of the matrix. In particular, \cite{Gopalan2014} and \cite{Zhou2015} considered a model based on the gamma process where
\begin{equation}
A_{ij}\sim \Poisson \left  (\sum_{k=1}^\infty r_k v_{ik}v_{jk}\right ),~1\leq i,j\leq n
\end{equation}
where the the positive weights $(r_k)_{k=1,\ldots,\infty}$ represent the importance of community $k$, and $v_{ik}>0$ represents the level of affiliation of individual $i$ to community $k$. \cite{Gopalan2014} and \cite{Zhou2015} assume that the weights $(r_k)$ are the jumps of a gamma process, ensuring the sum is almost surely finite. Using properties of Poisson random variables, the model can be equivalently represented as
\begin{align}
A_{ij}&=\sum_{k=1}^{\infty} Z_{ijk}\\
Z_{ijk}&\sim \Poisson(r_k v_{ik}v_{jk})
\end{align}
The latent variables $Z_{ijk}$ may be interpreted as the number of latent interactions between two individuals $i$ and $j$ with respect to community $k$, the overall number $A_{ij}$ of interactions being the sum of those community interactions. For example, two members of the same company who also play sport together may meet five times at the company, and twice at the sport center, resulting in seven interactions overall. \cite{Zhou2015} refers to the partition of $A_{ij}$ in terms of $Z_{ijk}$ as edge partition model. The overall number
\begin{equation}
K_n=\sum_{1\leq i, j\leq n}1_{Z_{ijk}>0}
\end{equation} 
of communities $k$ that generated at least one interaction between the $n$ individuals is termed the number of active communities. For the gamma process edge-partition model~\citep{Zhou2015}, the number of active communities $K_n$ grows logarithmically with the number $n$ of individuals.


The logarithmic assumption may be too restrictive. For example, the number of active features may be indeed unknown but bounded. Alternatively, the number of active features may increase at a superlogartithmic rate. In this paper, we consider extensions to the gamma process factorization model by considering that $(r_k)$ are the points of Poisson point process with L\'evy measure $\rho$. Depending on the property of the underlying measure, the model can deal with Poisson factorization models where the number of active features is (i) bounded, with a random upper bound, (ii) unbounded where the number of active features can increase as $\log(n)$ or $n^{2\sigma}$, for $\sigma\in(0,1)$. We focus in particular on the generalized gamma process where a single parameter $\sigma\in(-\infty,1)$ controls all three behaviors. 

The article is organized as follows. In Section 




%
%   Related to NMF are Poisson factor models, introduced by \citep{Dunson2005}, where a count data matrix  (Bayesian) NMF has found many applications in network analysis, signal processing or  The matrix may correspond to interactions between individuals  have been extensively studied as they provide a powerful tool to find latent structures. In the Poisson factor analysis setting, we observe a count data $A \in \mathbb{N}^{n\times m}$, and assume that it is a realization of a Poisson random matrix with unknown mean $\Lambda$, that we want to estimate and factorize.  A non negative factorization of $\Lambda$ can be interpreted as a latent membership assignment and hence give valuable insight about the hidden structure behind the data in addition to a strong predictive tool. In a recommendation system problem, this data can represent the history of ratings or purchases of $m$ items by $n$ clients. Then, such model allows to uncover latent features (\cite{canny2004gap},\cite{dunson2005bayesian}, etc.). In a network problem, taking $m=n$, the matrix can represent the interactions between $n$ users (emails sent for example). Therefore, such models can be used for overlapping community detection  (\cite{psorakis2011overlapping} ). In this work, we will present a probabilistic model with interpretable parameters that allows us to efficiently recover the latent structures but also predict missing entries.
%
%Bayesian models offer a flexible framework with interpretable parameters. In the community detection paradigm for example, on can cite the popular stochastic block model and its generalizations to overlapping communities (\cite{holland1983stochastic}, \cite{kemp2006learning}). However, one limitation of such models is that the user has to specify $K$ the number of communities/features. Here, we are interested in models where $K$ can be inferred from the observations and where it can grow potentially without an upper bound when the size of the network is increasing. In order to be able to infer the number of features or communities from the data, Bayesian non parametric (BNP) models have been used with success. In these models, latent structures are represented using a completely random measure (CRM, see \cite{kingman1967completely}) which are atomic. Each atom represents a latent feature. Therefore, having an infinite number of atoms leads to an unbounded number of features.
%In the recommendation system paradigm for example, the authors of \cite{paisley2009nonparametric} use the Beta process whereas in \cite{gopalan2014bayesian}, the authors use the Gamma process (GP). In the community detection problem, \cite{acharya2015nonparametric}, \cite{zhou2015infinite} also represent the latent communities through a Gamma Process. However, in all of these models, in order to be able able to do the inference, finite atom approximations have been used so far, which imposes a bound on the number of features or communities. In the recent work \cite{ohama2017model}, the authors build on \cite{zhou2015infinite} to propose a constrained model without truncation on the number of atoms by marginalizing the CRM. In that model, the communities are still represented by a Gamma process.
%
%
%
%In this work, we will mainly focus on overlapping communities detection (extension of the model to the recommendation system setting is left in Appendix). There has been an increasing interest on detecting communities within graphs. Hence, several algorithms and models have been studied, one can refer to \cite{fortunato2010community} and \cite{xie2013overlapping} for a review of the state of the art methods.
%
%
%%However, it is not always simple to define what a community is, specially when overlapping is allowed. Among the Bayesian methods, one can distinguish two approaches. The first one is to suppose that each node is affiliated to only one or a portion of the communities. Therefore, communities are defined as a clustering or feature allocation of the nodes. It is the case for instance for the stochastic block model (SBM, \cite{holland1983stochastic},\cite{kemp2006learning}). As explained in \cite{zhou2015infinite}, another approach is to suppose that every node is affiliated to all communities but with a different intensity. Then, the communities are defined as a clustering of the edges. These models are referred to as Edge Partition Models (EPM). In this work, we consider the latter approach.
%
%
%The data considered will represent directed integer valued weighted graphs as well as directed unweighted graphs. We will first show how the properties of the CRM relate to the number of communities and other properties of the graph. As a particular case, we show how the choice of the Gamma Process will impose some key asymptotic properties of the graph. Therefore, we present a MCMC algorithm for the more flexible class of the Generalized Gamma Process CRMs. We use slice variables in order to avoid approximations, therefore the model presented is "truly infinite". We show how to detect communities but also how to predict missing entries. Finally, the algorithm iterates only over the non zero entries of $A$, and hence, it takes advantage of the sparsity of the graph.  Indeed each iteration scales in $O(S K_+ )$ where $S$ is the number of non-zero entries of the adjacency matrix $A$, and $K_+$ the current estimation of the number of communities.
%
%\subsection*{Poisson factorization model}
%Let us consider a given directed weighted graph with $n$ nodes and integer valued weights. We represent this graph through its adjacency matrix $A = (A_{i,j})_{1 \leq i,j \leq n}$ where for all $(i,j)$, $A_{i,j}$ represents the weight of the directed edge from the node $i$ to the node $j$. We will abuse notation and identify a graph by its adjacency matrix. The objective of this work is to decompose the original graph into partial graphs with adjacency matrices $Z_{k}= (Z_{k,i,j})_{1 \leq i,j \leq n}$ which superposition gives $A$, meaning that
%$$A = \sum_k Z_{k}.$$
%Building on the countable additivity of Poisson random variables (see \cite{kingman1967completely}, chapter 1 for instance), one of the most popular ways to model such a structure is to suppose that $A_{i,j} \sim Pois(\Lambda_{i,j})$ and $Z_{k,i,j} \sim Pois(\lambda_{k,i,j})$, leading to
%$$ \Lambda_{i,j} = \sum_k \lambda_{k,i,j}.$$
%Of course, such an additive model is a simplification of reality. Nevertheless, it has proven through the years to give satisfactory results. \\
%
%To make the description of this setting more concrete, let us consider a particular example that we will keep through all this paper as illustration. Hence, let us suppose that $A$ represents a network of $n$ individuals where for instance $A_{i,j}$ is equal to the number of emails sent by $i$ to $j$. In this paradigm, we suppose that there are communities indexed by $k \in \mathbb{N}$. To each community $k$, a graph $Z_k$ is associated, where $Z_{k,i,j}$ is the number of emails sent by $i$ to $j$ and that are about or somehow associated with community $k$. Therefore
%$$ A_{i,j} = \sum_k Z_{k,i,j}.$$
%As mentioned in the previous paragraph, $Z_{k,i,j}$ follows a Poisson distribution with parameter $\lambda_{k,i,j}$. The idea here is to decompose such parameter into 3 parts. First, there should be a component that would encapsulate the overall activity of the community $k$ considered, or in other words the overall tendency of sending emails within community $k$. We will denote such a component $r_k$ (only depending on the community considered). The second and third parts quantify the 'affiliation' of $i$ and $j$ to community $k$, or their degree of commitment to that particular community. We will denote these quantities respectively $v_{k,i}$ and $v_{k,j}$. The desired behavior of $\lambda_{k,i,j}$ is to grow with all three of these parameters, therefore we will simply take:
%$$\lambda_{k,i,j} = r_k v_{k,i} v_{k,j}.$$
%Such decompositions are usually referred to as Poisson factorizations models, and have been successfully used for community detection, as in \cite{ball2011efficient} for instance.

